Zero-Shot Metric Depth with a Field-of-View Conditioned Diffusion Model

While methods for monocular depth estimation have made significant strides on standard benchmarks, zero-shot metric depth estimation remains unsolved. Challenges include the joint modeling of indoor and outdoor scenes, which often exhibit significantly different distributions of RGB and depth, and the depth-scale ambiguity due to unknown camera intrinsics. Recent work has proposed specialized multi-head architectures for jointly modeling indoor and outdoor scenes. In contrast, we advocate a generic, task-agnostic diffusion model, with several advancements such as log-scale depth parameterization to enable joint modeling of indoor and outdoor scenes, conditioning on the field-of-view (FOV) to handle scale ambiguity and synthetically augmenting FOV during training to generalize beyond the limited camera intrinsics in training datasets. Furthermore, by employing a more diverse training mixture than is common, and an efficient diffusion parameterization, our method, DMD (Diffusion for Metric Depth) achieves a 25\% reduction in relative error (REL) on zero-shot indoor and 33\% reduction on zero-shot outdoor datasets over the current SOTA using only a small number of denoising steps. For an overview see https://diffusion-vision.github.io/dmd

==> figures/fov_sweep.tex <==
\begin{figure*}[!h]
    \centering
    \scriptsize
    \setlength\tabcolsep{1pt} % default value: 6pt
    \newcommand{\Figwidth}{0.45\linewidth}
    \begin{tabular}{cc}
      Indoors & Outdoors \\
    \includegraphics[width=\Figwidth]{figures/fov_sweep/ibims1.png} &
        \includegraphics[width=\Figwidth]{figures/fov_sweep/vkitti2.png} \\
    \underline{ibims-1} & \underline{Virtual KITTI 2} \\
    \includegraphics[width=\Figwidth]{figures/fov_sweep/diode_indoor.png} &
    \includegraphics[width=\Figwidth]{figures/fov_sweep/diml_outdoor.png} \\
    \underline{DIODE Indoor} & \underline{DIML Outdoor} \\
    \includegraphics[width=\Figwidth]{figures/fov_sweep/hypersim.png} &
    \includegraphics[width=\Figwidth]{figures/fov_sweep/ddad.png} \\
    \underline{Hypersim} & \underline{DDAD} \\
        \end{tabular}
        \vspace*{-0.1cm}
	\caption{Plots showing changes in relative error on datasets \textbf{not seen during training} as we sweep over the field-of-view (fov) during evaluation. Despite not having seen these datasets during training, the optimal fov is close to the true fov. \srbs{may be just keep 3 with diverse fov}} \srbs{Why is there a bias?} \srbs{Use degrees instead of tan theta in plots?}
    \label{fig:fov_sweep}
    \vspace{-1em}
\end{figure*}


==> figures/log_depth_plot.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.32\textwidth]{figures/log_depth_plot.png}
\vspace*{-0.2cm}
\caption{Modelling depth in the log space allows allocating more representation capacity to regions with smaller depths, say $<$10 meters (shown by shaded region), which improves both qualitative and quantitative performance on such regions.
\ds{What does the purple region mean?}\srbs{Updated caption.}
\df{not clear a fig is nec for this?}\srbs{Keeping here for now, but can move to appendix if we need more space.}
}
\label{fig:log_depth_plot}
\end{figure}

==> tables/ablation_crop.tex <==
\begin{table*}[h]
\footnotesize
\centering
\setlength{\tabcolsep}{2.5pt} % cols space (default: 6pt)
\begin{tabular}{lccccc|ccccc}
\toprule
& \multicolumn{5}{c|}{\textbf{Indoors}} & \multicolumn{5}{c}{\textbf{Outdoors}} \\
Experiment & NYU & SunRGBD & DIODE Indoor & ibims-1 & Hypersim & KITTI & DIML Outdoor & DIODE Outdoor & Virtual KITTI 2 & DDAD \\
\midrule
No Crop or Uncrop & \textbf{0.074} & 0.124 & 0.337 & 0.180 & 0.479 & 0.055 & 1.399 & \textbf{0.615} & 0.095 & 0.116 \\
With Crop + FOV cond & 0.076 & \textbf{0.104} & \textbf{0.302} & \textbf{0.138} & \textbf{0.381} & \textbf{0.054} & \textbf{0.878} & 0.657 & \textbf{0.091} & 0.121 \\
\midrule
\% change & +2.70\% & -16.13\% & -10.39\% & -23.33\% & -20.46\% & -1.82\% & -37.24\% & 6.83\% & -4.21\% & +4.31\% \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Ablation showing the impact of cropping augmentation. We report the relative error.
\df{let's combine Tables 11 and 12 on crop/uncrop augmentations?}\srbs{Sounds good, will do.}
}
\label{tab:ablation-crop}
\end{table*}

==> tables/ablation_fov.tex <==
\begin{table*}[!htb]
\footnotesize
\centering
\setlength{\tabcolsep}{2.5pt} % cols space (default: 6pt)
\begin{tabular}{lccccc|ccccc}
\toprule
& \multicolumn{5}{c|}{\textbf{Indoors}} & \multicolumn{5}{c}{\textbf{Outdoors}} \\
Experiment & NYU & SunRGBD & DIODE Indoor & ibims-1 & Hypersim & KITTI & DIML Outdoor & DIODE Outdoor & Virtual KITTI 2 & DDAD \\
\midrule
No fov aug & \textbf{0.074} & 0.124 & 0.337 & 0.180 & 0.479 & \textbf{0.055} & 1.399 & 0.615 & 0.095 & \textbf{0.095} \\
Fov aug, no fov cond & 0.081 & 0.116 & 0.316 & 0.180 & 0.400 & 0.057 & 1.257 & \textbf{0.613} & 0.100 & 0.099 \\
Fov aug, fov cond & 0.076 & \textbf{0.109} & \textbf{0.298} & \textbf{0.130} & \textbf{0.382} & \textbf{0.055} & \textbf{0.300} & 0.628 & \textbf{0.093} & 0.101 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Ablation showing impact of field-of-view augmentation and conditioning. We report the relative error.}
\label{tab:ablation-fov}
\end{table*}

==> tables/ablation_num_steps.tex <==
\begin{table}[h!]
\footnotesize
\setlength{\tabcolsep}{3pt} % cols space
\centering
\begin{tabular}{c|cc}
\toprule

num\_steps & NYU   & KITTI \\ \midrule

1 & 0.079 & 0.056 \\
2 & 0.077 & 0.055 \\
4 & 0.076 & 0.055 \\
8 & 0.076 & 0.055 \\
16 & 0.076 & 0.055 \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Our model achieves good performance even with one denoising step. We report relative error. \srbs{Show plot instead?} \ds{It seems that more steps don't add much, was that observed for v-param on other tasks?} }
\label{tab:ablation-num-steps}
\end{table}

==> tables/ablation_uncrop.tex <==
\begin{table*}[!htb]
\footnotesize
\centering
\setlength{\tabcolsep}{2.5pt} % cols space (default: 6pt)
\begin{tabular}{lccccc|ccccc}
\toprule
& \multicolumn{5}{c|}{\textbf{Indoors}} & \multicolumn{5}{c}{\textbf{Outdoors}} \\
Experiment & NYU & SunRGBD & DIODE Indoor & ibims-1 & Hypersim & KITTI & DIML Outdoor & DIODE Outdoor & Virtual KITTI 2 & DDAD \\
\midrule
% Baseline & \textbf{0.074} & 0.124 & 0.337 & 0.180 & 0.479 & \underline{0.055} & 1.399 & \textbf{0.615} & 0.095 & \textbf{0.095} \\
Crop + FOV cond &  \textbf{0.076} & \textbf{0.104} & 0.302 & 0.138 & \textbf{0.381} & \textbf{0.054} & 0.878 & 0.657 & \textbf{0.091} & 0.121 \\
Crop \& Uncrop + FOV cond &  \textbf{0.076} & 0.109 & \textbf{0.298} & \textbf{0.130} & 0.382 & 0.055 & \textbf{0.300} & \textbf{0.628} & 0.093 & 0.122 \\
\midrule
\% change & 0.00\%  & +4.81\% & -1.32\% & -5.80\% & +0.26\% & +1.85\% & -65.83\% & -4.41\% & +2.20\% & +0.83\% \\
\bottomrule
\end{tabular}
\vspace{-6pt}
\caption{Ablation showing impact of uncropping augmentation. We report the relative error.}
\label{tab:ablation-uncrop}
\end{table*}

==> tables/results_kitti.tex <==
\begin{table}[t]
    \centering
    \scriptsize

    \setlength{\tabcolsep}{1pt}
    % \begin{tabularx}{0.98\linewidth}{l @{\hskip 0pt} l @{\hskip 0em} c @{\hskip 0em} ccccccc}
    \begin{tabular}{lcccccccc}
       \toprule
        Method & ~~~\textbf{$\delta_1$}$\uparrow$~~~ & ~~~\textbf{$\delta_2$}$\uparrow$~~~ & ~~~\textbf{$\delta_3$}$\uparrow$~~~ & ~REL~$\downarrow$~ & Sq-rel~$\downarrow$ & RMS~$\downarrow$ & RMS log~$\downarrow$ \\
        \midrule
       % Saxena~\etal~\cite{saxena2005learning} & - & 0.601 & 0.820  & 0.926 & 0.280   & 3.012  & 8.734 & 0.361    \\
       % Eigen~\etal~\cite{eigen2014depth} & Convolutions & 0.702 & 0.898 & 0.967 & 0.203   & 1.548  & 6.307 & 0.282    \\        % Liu~\etal~\cite{liu2015learning} & Convolutions & 0.680 & 0.898 & 0.967 & 0.201   & 1.584  & 6.471 & 0.273    \\
    %   Godard~\etal~\cite{godard2017unsupervised} & ResNet-50 & 0.861 & 0.949 & 0.976 & 0.114   & 0.898  & 4.935 & 0.206 \\
    %   Johnston~\etal~\cite{johnston2020self} & ResNet-101$^\dag$ & 0.889 & 0.962 & 0.982 & 0.106 & 0.861 & 4.699 & 0.185 \\
    %   Gan~\etal~\cite{gan2018monocular} & ResNet-101 & 0.890 & 0.964 & 0.985 & 0.098   & 0.666  & 3.933 & 0.173 \\
      % PLADE-Net~\cite{gonzalez2021plade} & FAL-Net & 0.900 & 0.967 & 0.985 & 0.089 & 0.590 & 4.008 & 0.172\\
    %   DORN \cite{dorn}  & ResNet-101$^\dag$ & 0.932 & 0.984 & 0.994 & 0.072   & 0.307  & 2.727 & 0.120\\
    %   VNL \cite{yin2019enforcing} & ResNext-101$^\dag$ & 0.938 & 0.990  & \third{0.998} & 0.072 & -- & 3.258 & 0.117 \\
    %   PGA-Net \cite{xu2020probabilistic} & ResNet-50$^\dag$ & 0.952 & 0.992 & \third{0.998} & 0.063 & 0.267 & 2.634 & 0.101 \\
    BTS \cite{bts} & 0.956 & 0.993 & {0.998} & 0.059   & 0.245  & 2.756 & 0.096 \\
    % TransDepth \cite{transdepth}  & 0.956 & 0.994 & {0.999} & 0.064 & 0.252  & 2.755 & 0.098 \\
    DPT \cite{dpt} & 0.959 & {0.995} & {0.999} & 0.062 & --& 2.573 & 0.092 \\
    AdaBins \cite{adabins} & 0.964 & {0.995} & {0.999} & 0.058  & 0.190  & 2.360 & 0.088\\
    BinsFormer \cite{binsformer} & {0.974} & {0.997} & {0.999} & {0.052} & {0.151} & {2.098} & {0.079} \\
    PixelFormer \cite{pixelformer} & {0.976} & {0.997}  & {0.999} & {0.051} & {0.149} & {2.081} & {0.077} \\
    MIM \cite{xie2022revealing} & {0.977} & {0.998} & {1.000} & {0.050} & {0.139} & {1.966} & {0.075} \\
    DDVM \cite{ddvm} &  0.965 &   0.994 &   {0.998}&   0.055 &   0.292 &   2.613 &   0.089 \\
    IEBins \cite{shao2023IEBins} & 0.978  & 0.998  & 0.999 & 0.050  &  0.142  &  2.011  & 0.075  \\
    \midrule
    ZoeD-M12-NK \cite{bhat2023zoedepth} &  0.966 &   0.993 &   0.996 &   0.057 &   0.204 &   2.362 &   0.087 \\
    \oursnk  & 0.964 & 0.994 & 0.999 & 0.055 & 0.219 & 2.527 & 0.087 \\
    \oursmix & 0.967  & 0.995 & 0.999 & 0.053 & 0.203  & 2.411 & 0.084 \\

\bottomrule
\end{tabular}
\vspace{-3pt}
\caption{\textbf{Comparison of performance on the KITTI dataset.} $\top$ indicates method uses unsupervised pretraining, \dag~indicates supervised pretraining and \ddag~indicates use of auxiliary supervised depth data. \textbf{Best} / \underline{second best} results are bolded / underlined respectively. $\downarrow$: lower is better and $\uparrow$: higher is better. \srbs{Add more recent baselines} \srbs{Put NYU and KITTI results side by side at the top}}
\label{tab:results-kitti}
\end{table} 

==> tables/results_nyu.tex <==
% Table from ZoeDepth

\begin{table}[t]
\centering
\footnotesize
%\begin{adjustbox}{\linewidth,center}
\begin{tabularx}{\linewidth}{@{}l*{5}{c}c@{}}
\toprule
\textbf{Method} &
\textbf{$\delta_1$}$\uparrow$       & \textbf{$\delta_2$}$\uparrow$          & \textbf{$\delta_3$}~$\uparrow$            & REL~$\downarrow$          & RMSE~$\downarrow$  & $\log_{10}$~$\downarrow$ \\ \midrule
% Eigen~\etal~\cite{eigen2014depth}    & 0.769          & 0.950          & 0.988          & 0.158            & 0.641          & --              \\  
% Laina~\etal~\cite{laina2016deeper}& 0.811          & 0.953          & 0.988          & 0.127            & 0.573          & 0.055                \\
% Hao~\etal~\cite{hao2018detail}        & 0.841          & 0.966          & 0.991          & 0.127            & 0.555          & 0.053                \\ 
% DORN~\cite{dorn}   & 0.828          & 0.965          & 0.992          & 0.115            & 0.509          &   0.051  \\
% SharpNet~\cite{ramamonjisoa2019sharpnet}          & 0.836          & 0.966          & 0.993          & 0.139            & 0.502          &      {0.047}          \\
% Hu~\etal~\cite{hu2019revisiting}        & 0.866          & 0.975          & 0.993          & 0.115            & 0.530          &    0.050            \\ 
% Lee~\etal~\cite{lee2019monocular}    & 0.837          & 0.971          & 0.994          & 0.131            & 0.538          &   --  \\
% Chen~\etal~\cite{chen2019structure}        & 0.878          & 0.977          & 0.994          & 0.111            & 0.514          &  0.048              \\ 
BTS~\cite{bts}& {0.885}          & 0.978          & 0.994          & 0.110            & {0.392}          & {0.047}          \\ 
% Yin~\etal~\cite{yin2019enforcing}   & 0.875          & 0.976          & 0.994          & {0.108}            & 0.416          & 0.048               \\ 
AdaBins~\cite{adabins} & {0.903} & {0.984} & {0.997} & {0.103}     & {0.364} & {0.044} \\ 
{LocalBins~\cite{bhat2022localbins}}  & {0.907} & {0.987} & \underline{0.998} & {0.099}     & {0.357} & {0.042} \\ 
Jun~\etal~\cite{jun2022depth}  & 0.913 & 0.987 & \underline{0.998} & {0.098}     & {0.355} & {0.042} \\ 
{NeWCRFs~\cite{yuan2022new}}  & 0.922 & \underline{0.992} & \underline{0.998} & {0.095}     & {0.334} & {0.041} \\ 
IEBins \cite{shao2023IEBins} & 0.936 &  0.992 &  0.998 & 0.087  &  0.314 & 0.038 \\
        % {TransDepth \citep{transdepth}} & 0.900 & 0.983 & 0.996 & 0.106 & 0.365 & 0.045\\
        {DPT \citep{dpt}} & 0.904 & 0.988 & \underline{0.998} & 0.110 & 0.357 & 0.045 \\
        {AdaBins \citep{adabins}} & 0.903 & 0.984 & \third{0.997} & 0.103 & 0.364 & 0.044 \\
        {BinsFormer \citep{binsformer}} & 0.925 & 0.989 & \third{0.997} & 0.094 & 0.330 & 0.040 \\
        {PixelFormer \citep{pixelformer}} & 0.929 & \third{0.991} & \underline{0.998} & 0.090 & 0.322 & 0.039 \\
        {MIM \citep{xie2022revealing}} & \underline{0.949} & \first{0.994} & \first{0.999} & 0.083 & \second{0.287} & \third{0.035} \\
        DDVM \cite{ddvm} & \third{0.946} & 0.987 & 0.996 & \first{0.074} & 0.315 & \first{0.032} \\
% \midrule
% \textbf{ZoeD-X-N}   & 0.946 & \underline{0.994} & \textbf{0.999} & {0.082}     & 0.294 & 0.035 \\
% \textbf{ZoeD-M12-N}  & \textbf{0.955} & \textbf{0.995} & \textbf{0.999} & \textbf{0.075}     & \textbf{0.270} & \textbf{0.032} \\ 
\midrule
ZoeD-M12-NK  & \textbf{0.953} & \textbf{0.995} & \textbf{0.999} & 0.077 & \textbf{0.277} & \underline{0.033} \\ 
\midrule
\textbf{\oursnk}  & \underline{0.944} & 0.986 & 0.996 & \underline{0.076} & 0.313 & \underline{0.033} \\
\textbf{\oursmix}  & \textbf{0.953} & 0.989 & 0.996 & \textbf{0.072} & \underline{0.296} & \textbf{0.031} \\

\bottomrule
\end{tabularx}
%\end{adjustbox}
\vspace{-3pt}
\caption{\textbf{Quantitative comparison on NYU-Depth v2.} The reported numbers of prior art are from the corresponding original papers. Best results are in bold, second best are underlined.  \ds{Use the same highlighting method as before.}}
%
\label{tab:results-nyu}
\end{table}
